Tunable Nanoparticle Stripe Patterns at Inclined Surfaces

Periodic assemblies of nanoparticles are central to surface patterning, with applications in biosensing, energy conversion, and nanofabrication. Evaporation of colloidal droplets on substrates provides a simple yet effective route to achieve such assemblies. This work reports the first experimental demonstration of patterns formed through stick-slip dynamics of the three-phase contact line during evaporation of gold nanoparticle suspensions on inclined substrates. Variation in nanoparticle concentration and substrate inclination alter the balance of interfacial and gravitational forces, producing multiple stick-slip events that generate periodic stripes. Stripe density exhibits a sinusoidal dependence on inclination angle, while inter-stripe spacing remains nearly invariant. Independent control over inter-stripe spacing is achieved through adjustment of nanoparticle or surfactant concentration. These results highlight the complex interplay of gravitational and interfacial forces in directing periodic nanoparticle assembly and establish a versatile, programmable framework for surface patterning with tunable nano/microscale dimensions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
